A Novel Metric for Measuring the Robustness of Large Language Models in Non-adversarial Scenarios

We evaluate the robustness of several large language models on multiple datasets. Robustness here refers to the relative insensitivity of the model's answers to meaning-preserving variants of their input. Benchmark datasets are constructed by introducing naturally-occurring, non-malicious perturbations, or by generating semantically equivalent paraphrases of input questions or statements. We further propose a novel metric for assessing a model robustness, and demonstrate its benefits in the non-adversarial scenario by empirical evaluation of several models on the created datasets.

==> chapters/back/benchmarking-results.back.tex <==
\section{Benchmarking Model Robustness}
\label{sec:benchmarking-experiments}
\subsection{Introduction
\label{ssec:metric_introduction}}

Consider $x_{i,0}$ and $(x_{i,1},\dots,x_{i,n(i)})$, the $\nth{i}$ original input and its $n(i)$ perturbations, in the perturbed dataset $D'$ (see Section~\ref{ssec:input_perturbations}).  Let $s_{i,0}$ and $(s_{i,1},\dots,s_{i,n(i)})$ be binary-valued scores (e.g., exact or string containment match) of the ground truth reference to the model's predicted value (e.g., generated answer) on the original and perturbed instances, respectively.  Let $p_{i,0}=s_{i,0}$ and $p_{i,1}=\frac{1}{n(i)}\sum_{j=1}^{n(i)}s_{i,j}$ be the average scores on the original and perturbed instances, respectively.  

We have defined a model's performance on a dataset as being \emph{robust} if the performance tends to be insensitive to perturbations; this is measured by the tendency for $p_{1,i}$ to be close to $p_{0,i}$, across instances $i$.  This is different from the model's performance overall, which would assess the averages of the scores (either original, perturbed, or both).  A model can be robust but have poor performance, or have high average performance on the original instances ($p_{i,0}$) but perform poorly on perturbations ($p_{i,1}$), making it non-robust.  In this we differ from \emph{worst-case} definitions of robustness (e.g., \citet[p. 133]{HELM}, \citet{wang-etal-2023-recode}), where a model must score correctly on all perturbed instances (e.g., $s_{i,j}=1,\:\forall j=1,\dots,n(i)$) to be considered robust.

We now describe the metrics we use to measure model performance robustness.  The metrics and instance scoring functions are implemented in the open-source repository \texttt{unitxt} \cite{unitxt}.  A given metric $f$ produces a group-level score $m_i=f(s_{i,0},s_{i,1},\dots,s_{i,n(i)})$. Thus, we have instance-group scores $(m_1,\dots,m_n)$ on $D'$. Statistical analysis of the metric is done by constructing 95\% bootstrapped confidence intervals on the $m_i$ scores, discarding any undefined values, rather than resampling the instance scores, reforming the groups, and calculating the group scores (which may be undefined if $s_{i,0}$ is missing).  This is is because we analyze the typical average robustness across original instances, and thus the unit of analysis is the original instance \emph{together with} its perturbations, as reflected in $m_i$.
%Our analysis aims to estimate the range of the metric value (in particular, the change in score after perturbation) that is expected across original instances $x_i\in D$ when they are perturbed.  Thus, the relevant observational unit is the \emph{group} an original instance $x_{i,0}\in D'$, \emph{together} with its perturbations $(x_{i,1},\dots,x_{i,n(i)})$---reflected in its metric value $m_i$---rather than individual instances $x\in D'$.  For this reason, we resample the group-level scores $(m_1,\dots,m_n)$, rather than resampling the instance scores $s_{i,j}$, re-forming the groups (which may now have duplicate instances or be incomplete in that the original score $s_{0,i}$ is missing) and calculating group-level metric values $m$ on them.


\subsection{Robustness Metrics}

%\ella{evaluation metrics: aggregation metrics (cohen’s h, abs(cohen’s h)): RPD cannot easily apply to cases where the ground truth is 0, statistically-sound metric, for cases where the ground truth is 1, it almost perfectly correlates with RPD (i.e., intuitive)}

\subsubsection{Performance Drop Rate (PDR)
\label{sssec:pdr}}

PDR \cite{promptBench_performance_drop_rate} is the fractional drop in the perturbed score average relative to the original baseline.  It is defined as
\[
\textrm{PDR}(p_{i,0},\:p_{i,1})=\begin{cases}
0, & p_{i,0}=p_{i,1}=0\\
\textrm{undefined}, & p_{i,0}=0, p_{i,1}\ne 0\\
1-\frac{p_{i,1}}{p_{i,0}}, & \textrm{otherwise}
\end{cases}
\]
The first case is added to the authors' definition.  PDR has an intuitive interpretation but no inherent thresholds indicating statistically-significant change relative to 0, the no-change value.  Also, it is undefined when the perturbations actually increase performance relative to a 0-value original score, a case that hopefully should be uncommon.

\subsubsection{Cohen's $h$ Effect Size
\label{sssec:cohens_h_effect_size}
}

We use Cohen's $h$ \cite{C1988} statistical effect size metric for the difference in proportions (see Appendix~\ref{sec:appendix} for background), defined as
\[
\CoH{p_{i,0}}{p_{i,1}}=2\left(\arcsin{(\sqrt{p_{i,1}})}- \arcsin{(\sqrt{p_{i,0}})}\right)
\]
Cohen's $h$ has several important features:
\begin{itemize}[leftmargin=*]
    \item Unlike PDR, it is a symmetric function, and is defined for all valid values $p_{i,0},p_{i,1}\in[0,1]$.
    \item It has rule-of-thumb thresholds (\citet{C1988}, \citet{S2009}) of a statistically-significant difference in sample proportions, which are based on statistical properties:
    $|h|<0.01$ (essentially zero); $0.01\leq |h| < 0.2$ (very small); $0.2 \leq |h| < 0.5$ (small); $0.5\leq |h|<0.8$ (medium); $0.8 \leq |h| < 1.2$ (large); $1.2 \leq |h| < 2.0$ (very large); $2.0 \leq |h|$ (huge).
\end{itemize}

Cohen's $h$ takes values in the range $[-\pi, \pi]$.
%since $\arcsin{(1)}=\pi/2$ and $\arcsin{(0)}=0$.  
For better interpretability, we define its normalization
\[\NCoH{p_{i,0}}{p_{i,1}}=\CoH{p_{i,0}}{p_{i,1}}/\pi
\]
\noindent which takes values in $[-1,1]$; its significance thresholds are the ones above, each divided by $\pi$.  
%Being a constant normalization, $\NCoHfunc$ inherits all other properties of $H$.  
We also define its absolute value
\[
\ANCoH{p_{i,0}}{p_{i,1}}=
|\NCoH{p_{i,0}}{p_{i,1}}|
\]
$\ANCoHfunc$ measures change in either direction, and when its average and confidence interval are calculated on the dataset $D'$, it can serve as a proxy for the expected variance or absolute deviation between the original and perturbed instance performance.

Figure~\ref{fig:pdr_cohensh} compares $\NCoHfunc$ and `reverse PDR' ($=-1\times\textrm{PDR}$) when the original instance accuracy is $p_{i,0}$ is perfect (1.0).  Note that in this case, both metrics take values in $[-1,0]$ and have high visual correlation, indicating that $\NCoHfunc$---a statistical distribution-based metric---gives similar results to PDR, which is inherently interpretable since it involves percentage change.
For a fixed $|p_{i,0}-p_{i,1}|$, $|\NCoH{p_{i,0}}{p_{i,1}}|$ grows the closer one of the proportions is to 0 or 1, because these cases reduce the estimated pooled sample variance, making the difference between $(p_{i,0},p_{i,1})$ more statistically significant. 
Thus, for a fixed $p_{i,0}$, $\NCoH{p_{i,0}}{p_{i,1}}$ decreases non-linearly with changes in $p_{i,1}$, while PDR decreases linearly.  

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{robustness/figures/pdr_h_comparison.png}
\caption{Comparison of normalized Cohen's $h$ ($\NCoHfunc$) and reverse PDR (=$-1\times\textrm{PDR}$) when the original instance accuracy $p_{i,0}=1.0$.}
\label{fig:pdr_cohensh}
\end{figure}

When we calculate 95\% confidence intervals for $\NCoHfunc$, the interpretation is: if the entire interval is contained within the thresholds $\pm 0.2/\pi\approx \pm0.0637$ (`very small') or $\pm 0.5/\pi \approx \pm 0.1592$ (`small'), we can say that on any instance, the difference in performance from perturbation is likely to be marginal; if, in addition, the interval contains 0, the model can be considered more strictly robust in that there is plausibly no change in performance at all.

\subsection{Experimental Setup}

We conduct experiments using the following LLMs:

\begin{itemize}[leftmargin=*]
\item \textbf{Google Research}: Flan-T5-XXL (11B; \citet{chung2022scaling}) and Flan-UL2 (20B; \citet{flan_ul2}).
\item \textbf{IBM Research}: granite.13b versions chat-v2, instruct-v1, and instruct-v2 \cite{granite}.
\item \textbf{Meta}: Llama-2-chat 7B, 13B, and 70B \cite{touvron2023llama}; Llama-3-instruct 8B and 70B \cite{llama3}.
\item \textbf{Mistral AI}: mixtral-8x7b-instruct-v01 \cite{jiang2024mixtral}.
\end{itemize}

All results shown use zero-shot prediction and a temperature of 0.



%\ella{models, prompts, 0- or few-shot, etc.}

\subsection{Experimental Results}

%\ella{the main results of the paper -- robustness report (style what we have in the dashboard), some analyses, possibly charts}

Table~\ref{tab:overall_averages} shows the aggregate value of several summary metrics, where the mean is taken first across all instances in each perturbed dataset $D'$ (see Section~\ref{sec:dataset}), then the unweighted mean is taken across the datasets.  The table shows the aggregated mean score on the original unperturbed instances ($p_{i,0}$), and normalized Cohen's $h$ ($\NCoHfunc$) and its absolute value ($\ANCoHfunc$), comparing the original instance score to the pooled set of all perturbation variants regardless of type (see Section~\ref{ssec:input_perturbations}).  The best model result for each metric is bolded.  The Llama models and Mixtral tend to perform the best on the original instances, with the Llama-3-70B-instruct model (the largest) being the best, though only marginally better than the much smaller Mixtral model.  Overall, Flan-T5-XXL has the best perturbation robustness, as indicated by low values of both Cohen's $h$ metrics.  However, all models' aggregated $\NCoHfunc$ are within the bounds of a `very small' change vs the original (see Section~\ref{sssec:cohens_h_effect_size}), and all individual dataset averages (not shown here) are within the `small' change thresholds, indicating that they are all fairly robust on our perturbed datasets.  

\begin{table}
\hspace*{-1.8cm}
\begin{tabular}{l|rrr}
\hline
 model & $p_{i,0}$ & $\NCoHfunc$ & $\ANCoHfunc$ \\
 \hline
google/flan-t5-xxl & 0.677 & \bfseries -0.011 & \bfseries 0.059 \\
google/flan-ul2 & 0.708 & -0.022 & 0.062 \\
ibm/granite-13b-chat-v2 & 0.628 & -0.027 & 0.112 \\
ibm/granite-13b-instruct-v1 & 0.593 & -0.030 & 0.115 \\
ibm/granite-13b-instruct-v2 & 0.603 & -0.014 & 0.069 \\
meta-llama/llama-2-7b-chat & 0.660 & -0.024 & 0.094 \\
meta-llama/llama-2-13b-chat & 0.714 &  -0.044 & 0.111 \\
meta-llama/llama-2-70b-chat & 0.741 & -0.041 & 0.094 \\
meta-llama/llama-3-8b-instruct & 0.676 & -0.030 & 0.096 \\
meta-llama/llama-3-70b-instruct & \bfseries 0.750 & -0.025 & 0.081 \\
mistralai/mixtral-8x7b-instruct-v01 & 0.749 & -0.033 & 0.103 \\
\hline
\end{tabular}
\caption{\label{tab:overall_averages}
Aggregated model metric scores, averaged across instances then across datasets.  Shown are mean score on the original unperturbed instances ($p_{i,0}$), and normalized Cohen's $h$ ($\NCoHfunc$) and its absolute value ($\ANCoHfunc$) for all perturbations vs the original.
}
\end{table}

Figure~\ref{fig:metric_summary} shows the robustness metric values by model and dataset.  The bar colors represent the model source (Google, IBM, Meta, Mistral), while the individual models are distinguished by the diagonal hashing pattern.  At the top of each bar, a red line shows the 95\% bootstrapped confidence interval (see Section~\ref{ssec:metric_introduction}).    

The first line shows the average original ($p_{i,0}$) and perturbed ($p_{i,1}$) instance scores.  All models perform significantly worse on PopQA than on the other datasets, since it is an open-ended, rather than boolean, question-answering task.  The third plot shows normalized Cohen's $h$ ($\NCoHfunc$), with the horizontal blue line at $\NCoHfunc\approx-0.0637$, a `very small' decrease.
Here, the mean values are nearly always negative, since the perturbations decrease predictive performance; even so, nearly all of the decreases are firmly minor, less than `very small', or even approximately zero (stricter robustness).  This agrees with the fact that the confidence intervals for $p_{\cdot,0}$ and $p_{\cdot,1}$ tend to have significant overlap. The relative magnitudes of $\NCoHfunc$ and $\ANCoHfunc$ also correlate well with PDR, which, despite its drawbacks (see Section~\ref{sssec:pdr}), can serve as a good sanity check.

\begin{figure}[h!]
%\hspace*{1.5cm}
\centering
\includegraphics[width=1.2\linewidth]{robustness/figures/metric_summary.png}
\caption{Metric scores by model and dataset. Red error bars show a 95\% bootstrapped confidence interval.}
\label{fig:metric_summary}
\end{figure}






==> chapters/back/datasets.back.tex <==
\section{Datasets}
\label{sec:dataset}

\subsection{Dataset Descriptions
\label{ssec:dataset_descriptions}}

In our experiments, we use use several input datasets.  These are

\begin{itemize}[leftmargin=*]
    \item \textbf{PopQA} \cite{mallen2023not}: a dataset of free-response questions of a factual nature about public figures and entities (e.g., who is the director/screenwriter/author of a film or book, what is the occupation/birthplace of a public figure).  A generated answer is correct if any of the reference answers are a substring of it.
    \item \textbf{BOOLQ} \cite{clark2019boolq}: A dataset of difficult reading-comprehension questions with boolean answers.
    \item \textbf{SIGA} (Social Identity Group Abuse, \citet{wiegand-etal-2022-identifying}): A dataset of short statements.  The task is to identify if the statement is abusive towards a social group (e.g., by race, religion, gender identity) but which is implicit (does not contain an abusive word that can be easily identified as such by lookup in a lexical dataset).  An example of such a statement is "People from other cultures are not like us."
    \item \textbf{Social stigma}: A dataset of statements generated by Google's Flan-UL2 \cite{flan_ul2} model based on a seed of human-written ones.  The task is to predict if the statement contains a negative stigmatizing attitude towards a social group.
    % Similarly to SIGA,
    % this dataset contains short statements, and the task is to identify if the statement displays a negative sentiment (stigma) towards a particular social group or not (either a positive sentiment, or neither).  Examples are ``I don't want to be around immigrants" and ``People need to respect the cultures of others", respectively.  
    %Beginning with a seeding dataset of both human-written and model-generated statements, samples from the seed dataset were used as context for a prompt to Google's Flan-UL2 \cite{flan_ul2} model, to continue generating similar examples.  Both the original seed and subsequently-generated statements were human-labeled as to whether they contained a stigmatizing statement. See \citet{Nagireddy_Chiazor_Singh_Baldini_2024} for similar use of social stigma in NLP.
    %\item \textbf{MMLU} (Measuring Massive Multitask Language Understanding; \cite{hendryckstest2021}, \cite{hendrycks2021ethics}): A dataset of multiple-choice standardized-test type questions on 57 subjects (e.g., mathematics, history, businesses, sciences). 
\end{itemize}

\subsection{Input Perturbations
\label{ssec:input_perturbations}}

In our experiments, the models receive input text that consists of 1) general instructions, 2) a question prompt, and 3) the question/statement itself.  For instance, for the social stigma dataset, the instructions explain what `social stigma' is, and the question prompt asks the model to answer with True/False whether the statement provided contains social stigma.  To test the robustness of the models, we perturb the question or statement only, leaving any instructions and question prompts unchanged. We use the following perturbation types, which are non-adversarial and imitate naturally-occurring variations:

\begin{itemize}[leftmargin=*]
    \item \textbf{superficial} (s): non-semantic perturbations, one of 1) capitalize all letters in the input;
    2) change the case of the first letter in the input; 3) replacing two instances of single spaces with five spaces; 4) removal of punctuation at the end of the input; or 5) "butterfingers" misspelling by replacing a randomly-selected letter with one of the adjacent ones on a keyboard.
    \item \textbf{distraction} (d): 
    \item \textbf{paraphrase} (p): On PopQA, we use manually-templated paraphrases created by \cite{rabinovich-etal-2023-predicting}, since all questions in a PopQA topic follow a single format.  For other datasets, up to 5 semantic paraphrases are generated using IBM's granite.13b.chat.v2 \cite{granite}, retaining only those with at least 0.7 cosine similarity with the original input.
    %an automatically-generated semantic paraphrase, created by \texttt{NL-Augmenter} \cite{dhole2021nlaugmenter}.
\end{itemize}

Table~\ref{tab:dataset_perturbations} summarizes the dataset task and the perturbation types used.  The perturbations are done to the test set of each dataset, not its training set.  Thus, let $D$ denote an unperturbed test dataset, consisting of $n$ unique instances $x_1,\dots,x_n$ (e.g., questions to be answered).  The perturbed dataset $D'$ consists of each original instance $x_i$ (now called $x_{i,0}$), as well as a random sample of $n(i) \geq 1$ perturbations of it, denoted $(x_{i,1},\dots,x_{i,n(i)})$.


\begin{table}[h!]
\centering
 \begin{tabular}{l |l l} 
 \hline
 Dataset & Task & Perturb.\\ 
 \hline
 PopQA & open answer & s/p \\
 BOOLQ & binary classification & s/p/d \\
 SIGA & binary classification & s/p \\
 Social Stigma & binary classification & s/p \\
 %MMLU & multiple-choice & p\\
 \hline
 \end{tabular}
\caption{Datasets and perturbation types  used (`s'=superficial; `p'=paraphrase; `d'=distraction).  
\label{tab:dataset_perturbations}}
\end{table}


%\ella{expanding existing datasets with naturally occurring variants for assessment of the robustness of LLMs; datasets (4+): will be open-sourced; perturbation generation – description and examples}
\\



\ella{need to justify the choice of these specific perturbations -- why not bias for instance (modifying "he" to "she", or replacing named entities)}


==> chapters/back/introduction.back.tex <==
\section{Introduction}
\label{sec:introduction}

With the increase in the prominence and use of large language models, there has been tremendous activity in evaluating various aspects of these models' behavior and aligning their behavior with desirable qualities.  For instance, assessing their privacy, safety, and accuracy.  One such desirable quality is \emph{robustness}, that is, their ability to generate consistent and equivalent outputs when given inputs that are essentially equivalent in the relevant domain.  Here, we assess the robustness of several state-of-the-art LLMs on question-answering and natural language classification tasks, by evaluating the models' accuracy when the inputs are perturbed in several meaning-preserving ways.  We use several perturbation types, both superficial (e.g., whitespace, letter case, punctuation) and semantic (paraphrasing), which together provide a more comprehensive assessment of the model's robustness.

Section~\ref{sec:rel-work} reviews related work on model robustness.  Section~\ref{sec:dataset} introduces the natural language datasets used, and the perturbations performed, on which robustness is assessed.  Section~\ref{sec:benchmarking-experiments} defines the metrics used to measure robustness. Section~\ref{sec:conclusions} concludes.  Section~\ref{sec:limitations} discusses limitations of this work.

This work makes several important contributions to the robustness analysis literature.  The first is that we use statistical effect size metrics to measure robustness, which we believe is a novel adaptation to this domain; as discussed in Section~\ref{sec:benchmarking-experiments}, these metrics have advantages over others used in the literature.  For all metrics used, we employ group-level bootstrapping to obtain confidence intervals to assess the robustness in terms of statistical significance of an observed accuracy change due to the perturbation.

==> chapters/back/related-work.tex <==
\section{Related Work}
\label{sec:rel-work}

%\ella{lot of work has been done on robustness... need to position our study in the broad context}

Generative LLMs cannot formally reason, but rather generate responses based on learned patterns in training data.  Thus, there is significant interest in whether their abilities are robust, or sensitive, to meaning-preserving perturbations of input.  Robustness is typically of interest either in evaluating a model's predictive ability on benchmark datasets constructed for the purpose, or in the training the model itself to be be more robust (e.g., \citet{zhao2024improving}), or both.

\citet{VWR2023} and \citet{mizrahi2024stateofwhat} show that LLMs are sensitive to prompt templates and instruction wording, and therefore propose using an ensemble of templates and prompts.  \citet{wang2023wordlevel} evaluate robustness of helpfulness and harmlessness LLM-as-a-judge scores in open-ended question-answering with word-level perturbations.  Naturally, the characterization of the robustness and the relevant perturbations depend on the domain and task.  In logical reasoning tasks, \citet{chen2024premise} investigate sensitivity to perturbing the order of logical premises.  In the code domain, the ReCode benchmark \citep{wang-etal-2023-recode} for Python function completion conducts meaning-preserving superficial (e.g., function name and docstring) and the documentation function examples, such as variable names (which require domain knowledge); these perturbations may affect the likelihood of generated code passing pre-defined unit tests.
